Variability Need Not Imply Error: The Case of Adequate but Semantically Distinct Responses

With the broader use of language models (LMs) comes the need to estimate their ability to respond reliably to prompts (e.g., are generated responses likely to be correct?). Uncertainty quantification tools (notions of confidence and entropy, i.a.) can be used to that end (e.g., to reject a response when the model is `uncertain'). For example, Kuhn et al. (semantic entropy; 2022b) regard semantic variation amongst sampled responses as evidence that the model `struggles' with the prompt and that the LM is likely to err. We argue that semantic variability need not imply error--this being especially intuitive in open-ended settings, where prompts elicit multiple adequate but semantically distinct responses. Hence, we propose to annotate sampled responses for their adequacy to the prompt (e.g., using a classifier) and estimate the Probability the model assigns to Adequate Responses (PROBAR), which we then regard as an indicator of the model's reliability at the instance level. We evaluate PROBAR as a measure of confidence in selective prediction with OPT models (in two QA datasets and in next-word prediction, for English) and find PROBAR to outperform semantic entropy across prompts with varying degrees of ambiguity/open-endedness.

==> old_experiments.tex <==
\section{Experiments}

% \subsection{Verify Semantic Entropy's limitation}
% \label{sec:exper_sem_ent}
We aim to assess how informative SE and \probar are in a setting where multiple semantically varying responses can be considered adequate. 
We conduct our experiments using a similar experimental setup to \citet{kuhn2022semantic} so as to ensure that the effects we observe are evidence consistent with our hypothesis, \emph{i.e.} SE is a poor predictor of correctness in the presence of data uncertainty.
To ensure that assessed prompts are open-ended 
%The original work, demonstrates the method's efficacy %in the task of QA, on two datasets: TriviaQA\cite{joshi2017triviaqa} and CoQA\cite{reddy2019coqa}. Both of these are general knowledge 
%on QA datasets where no or minimal data uncertainty is to be expected and a single ground truth generally exists.
%We seek to replace that with a task or dataset that exhibits data uncertainty;%, so as to demonstrate the failure of semantic entropy to correlate with correctness under such circumstances. For this reason, 
 we employ Abg-COQA \cite{guo2021abg} for our experiments---a reading comprehension QA dataset; where a passage is accompanied by one or more rounds of questions\footnote{Details on how the model prompt was constructed can be found in Appendix \ref{}}. More specifically, we focus on the subset of context-question pairs from the dataset where the last question is ambiguous, and given the passage, multiple answers (which are provided) are plausible (\Cref{fig:abg_coqa_example} shows an example). This comprises 994 context-ambiguous question pairs. %(741, 130 and 123 items from the training, development and testing sets respectively).

\begin{figure}[t]
    \begin{center}
        \includegraphics[width=7 cm]{latex/visuals/uncertainty-23.pdf}
        \caption{Example of an ambiguous instance from Abg-COQA.}  
        \label{fig:abg_coqa_example}
    \end{center}
\end{figure}

%The remaining components of the experimental setup remain similar to the original work. 
We evaluate on OPT models \cite{zhang2022opt}, varying in size --- 2.7B, 6.7B, 13B and 30B and we sample 10 unbiased generations per prompt. 
We evaluate using a selective generation setting, where the uncertainty indicator is informing a user as to whether they should rely on a model decision or abstain.
We operationalise it using Area Under the Receiver Operating Characteristic curve (AUROC). In essence, this is quantifying the probability that a randomly sampled correct response has a lower uncertainty score than a randomly sampled incorrect one. A higher score is desirable, with a perfect metric achieving an AUROC score of 1, and a random one would result in an AUROC of 0.5. 
We compare SE's and \probar's performance with PE. %of the Monte Carlo estimated distribution for $P(Y|X=x)$. 
However, we notice that when computing AUROC, we aggregate entropy values that do not share the same scale, as the number of elements in the distributions' support vary per instance (\emph{i.e.} the number of unique responses for PE and the number of clusters for SE). This might cause AUROC values to be misleading. We account for that by normalising entropy by its upper bound for every instance, and transforming it to a confidence score (\emph{i.e.} higher confidence score associated with higher correctness): $SE_{norm}(x) = 1-SE(x)/log(|C|)$ and $PE_{norm}(x) = 1-PE(x)/log(|N|)$. We compare \probar's AUROC scores to $SE_{norm}$'s and $PE_{norm}$'s.
Furthermore, we evaluate \probar, $SE_{norm}$ and $PE_{norm}$ (which are confidence-like scores) by visualising risk (fraction of false instances divided by number of predicted instances) versus coverage (fractions of predicted instances divided by all instances) plots.

\subsection{Idealised Conditions Evaluation}
Computing SE and \probar require parameterising functions that re-partition the space of responses to semantically equivalent or adequacy-related classes ($s(\cdot;\phi)$ and $a(\cdot;\lambda)$ respectively).%, both of which allow for algorithmic error. 

Initially, we evaluate the usefulness of these uncertainty indicators under idealised conditions ($s(\cdot;\phi)$ and $a(\cdot;\lambda)$ are perfect classifiers). Hence, we assess how useful these indicators are theoretically, while simultaneously estimating an upper bound on their performance.  
We randomly sample 50 context-ambiguous question pairs from the dataset's training set and manually annotate for the semantic equivalence and adequacy of the sampled responses and the mode. For adequacy, we annotate using finer-grained notions, as seen in \Cref{table:correctness_labels} of the Appendix, which are ultimately mapped to a binary adequacy decision --- used as correctness labels during evaluation. %, in an analysis similar to \Cref{sec:exper_sem_ent}.

\subsection{Realistic Conditions Evaluation}
We transfer our evaluation to a more realistic setting; we implement algorithms to automate the $s(\cdot;\phi)$ and $a(\cdot;\lambda)$ functions and the mode's correctness decision. 
To assess correctness automatically, we compute Rouge-L score \cite{lin2004automatic}, which measures the longest common subsequence, between the mode and any plausible answer (or a clarification question) and check whether it is higher than 0.3. 
For $s(\cdot;\phi)$, we use the algorithm described in \Cref{sec:background_measure_unc}, using Deberta-Large \cite{he2020deberta} as the NLI model. %assessing semantic equivalence.
For $a(\cdot;\lambda)$, we consider two approaches: %, whether the response is adequate for the prompt. In the case of the reading comprehension QA task, the response to the question will depend on the context given. %and should be consistent with that, rather than rely on the prompted model's own parametric memory.


%\subsection{Controlling for algorithmic error}
%In order to be able to obtain the clusters of sentences with equivalent meaning, the authors parameterise a clustering algorithm based on Natural Language Inference (NLI). Simultaneously, during evaluation, we assess the correctness of the greedy response as a decision made using an automated metric against an arbitrary threshold. 
%Both of these comprise sources of error. As a means to differentiate what part of the observed effects from experiments in \Cref{sec:exper_sem_ent} is due to the introduction of data uncertainty and which is due to such algorithmic errors, we conduct a controlled experiment. 




(1) \textbf{NLI model.} An NLI model is given as a premise the passage and as a hypothesis an affirmative sentence comprised from the question-response pair, generated using a LM. If the entailment probability %(\emph{i.e.} the sentence is supported by the context) 
is higher than the sum of probabilities of neutrality and contradiction, then the response is considered as adequate. %to the question (given the context), 
%and otherwise, it is considered inadequate.
We experiment with two NLI models: Deberta-Large \citep{he2020deberta}%, which was also used in the original work
, as well as Roberta-large, fine-tuned on a more challenging dataset collected via an iterative, adversarial human-and-model-in-the-loop procedure \citep{nie-etal-2020-adversarial}. The former method is referred to as NLI-Easy and the latter as NLI-Hard. To construct the affirmative sentence, Mistral-7B-Instruct-v0.2 \citep{jiang2023mistral} is used.

(2) \textbf{LM as classifier.} We prompt a LM to act as a classifier; it is given a document (context) and a claim (affirmative sentence created from a question response pair from a LM) and is prompted to generate True if the claim is supported by the passage, or False if not; referred as LM 2-Steps Support in experiments. Other prompt variations attempted include: including examples in the prompt (LM 2-Steps Few-Shot), adjusting wording where instead of seeking support for the claim, the task is weakened by simply asking whether the claim was not contradicted by the document (LM 2-Steps No Contradiction), and a version where instead of a claim, the original question-answer pair is used, eliminating the intermediate claim generation step (LM 1-Step). We use Mistral-7B-Instruct-v0.2 \citep{jiang2023mistral} for the claim generator and the LM classifier. Further details in the Appendix. 


\begin{figure*}
\hfill
\includegraphics[width=7.8cm]{latex/visuals/ambgcoqa_auroc_vs_model_manual_correct_chatgpt_as_judge_0-50_fewer_models.pdf}
\hfill
\includegraphics[width=7.8cm]{latex/visuals/ambgcoqa_auroc_vs_model_automatic_correct_chatgpt_as_judge_0-741_fewer_models.pdf}
\includegraphics[width=7.8cm]{latex/visuals/ambgcoqa_auc_vs_model_manual_correct_chatgpt_as_judge_0-50_fewer_models.pdf}
\hfill
\includegraphics[width=7.8cm]{latex/visuals/ambgcoqa_auc_vs_model_automatic_correct_chatgpt_as_judge_0-741_fewer_models.pdf}
\hfill
% \subfigure{\includegraphics[width=7.8cm]{latex/visuals/ambigqa_auroc_vs_model.pdf}}
% \hfill
\caption{AUROC values for different models under different uncertainty estimators. On the left, figure shows results under an automatic correctness decision for the greedy generation, while for the right figure, correctness was manually annotated.}
\label{fig:auroc_vs_model}
\end{figure*}

\begin{figure*}
\hfill
\includegraphics[width=7.8cm]{latex/visuals/ambgcoqa_auroc_vs_model_random_sample_manual_correct_chatgpt_as_judge_0-50_fewer_models.pdf}
\hfill
\includegraphics[width=7.8cm]{latex/visuals/ambgcoqa_auc_vs_model_random_sample_manual_correct_chatgpt_as_judge_0-50_fewer_models.pdf}
\caption{Avg AUROC and AUC values for 5 runs of different samples used as correctness criterion different models under different uncertainty estimators.}
\label{fig:auroc_vs_model}
\end{figure*}

\begin{figure*}
\hfill
\includegraphics[width=7.8cm]{latex/visuals/provo_corpus_auroc_vs_model_0-100.pdf}
\hfill
\includegraphics[width=7.8cm]{latex/visuals/provo_corpus_auc_vs_model_0-100.pdf}
\caption{AUROC and AUC values for different models under different uncertainty estimators for toy task.}
\label{fig:auroc_vs_model}
\end{figure*}

\begin{table*}[]
\scalebox{0.74}{
\begin{tabular}{l|ccccr|ccccr|ccccr}
                   & \multicolumn{5}{c|}{\textbf{NLI Easy}}                                                                                           & \multicolumn{5}{c|}{\textbf{NLI Hard}}                                                                               & \multicolumn{5}{c}{\textbf{LLM 1-Step}}                                                                                \\ \cline{2-16} 
                   & \textbf{2.7B} & \textbf{6.7B} & \textbf{13B} & \multicolumn{1}{c|}{\textbf{30B}}   & \multicolumn{1}{l|}{\textbf{Avg}}           & \textbf{2.7B} & \textbf{6.7B} & \textbf{13B} & \multicolumn{1}{c|}{\textbf{30B}} & \multicolumn{1}{l|}{\textbf{Avg}} & \textbf{2.7B}  & \textbf{6.7B} & \textbf{13B}   & \textbf{30B}                      & \multicolumn{1}{l}{\textbf{Avg}} \\ \hline
\textbf{Recall}    & 0.315         & 0.338         & 0.357        & \multicolumn{1}{c|}{0.300}          & 0.328                                       & 0.193         & 0.243         & 0.213        & \multicolumn{1}{c|}{0.203}        & 0.213                             & 0.740          & 0.684         & \textbf{0.799} & \multicolumn{1}{c|}{0.729}        & {\ul \textbf{0.738}}             \\
\textbf{Precision} & 0.679         & 0.740         & 0.792        & \multicolumn{1}{c|}{\textbf{0.816}} & {\color[HTML]{000000} {\ul \textbf{0.757}}} & 0.574         & 0.638         & 0.694        & \multicolumn{1}{c|}{0.730}        & 0.659                             & 0.709          & 0.731         & 0.757          & \multicolumn{1}{c|}{0.789}        & 0.746                            \\
\textbf{Accuracy}  & 0.698         & 0.672         & 0.654        & \multicolumn{1}{c|}{0.592}          & 0.654                                       & 0.656         & 0.624         & 0.586        & \multicolumn{1}{c|}{0.536}        & 0.601                             & \textbf{0.795} & 0.763         & 0.785          & \multicolumn{1}{c|}{0.752}        & {\ul \textbf{0.773}}             \\
\textbf{F1}        & 0.430         & 0.464         & 0.493        & \multicolumn{1}{c|}{0.440}          & 0.457                                       & 0.289         & 0.352         & 0.326        & \multicolumn{1}{c|}{0.318}        & 0.321                             & 0.724          & 0.707         & \textbf{0.778} & \multicolumn{1}{c|}{0.758}        & {\ul \textbf{0.742}}             \\
\textbf{}          & \multicolumn{5}{c|}{\textbf{LLM 2-Steps (Support)}}                                                                              & \multicolumn{5}{c|}{\textbf{LLM 2-Steps (No contradiction)}}                                                         & \multicolumn{5}{c}{\textbf{LLM 2-Steps (Few-Shot)}}                                                                    \\ \cline{2-16} 
\textbf{}          & \textbf{2.7B} & \textbf{6.7B} & \textbf{13B} & \multicolumn{1}{c|}{\textbf{30B}}   & \multicolumn{1}{l|}{\textbf{Avg}}           & \textbf{2.7B} & \textbf{6.7B} & \textbf{13B} & \multicolumn{1}{c|}{\textbf{30B}} & \multicolumn{1}{l|}{\textbf{Avg}} & \textbf{2.7B}  & \textbf{6.7B} & \textbf{13B}   & \multicolumn{1}{c|}{\textbf{30B}} & \multicolumn{1}{l}{\textbf{Avg}} \\ \hline
\textbf{Recall}    & 0.636         & 0.623         & 0.689        & \multicolumn{1}{c|}{0.632}          & 0.645                                       & 0.635         & 0.639         & 0.713        & \multicolumn{1}{c|}{0.651}        & 0.660                             & 0.587          & 0.633         & 0.627          & \multicolumn{1}{c|}{0.596}        & 0.611                            \\
\textbf{Precision} & 0.632         & 0.668         & 0.698        & \multicolumn{1}{c|}{0.750}          & 0.687                                       & 0.598         & 0.619         & 0.661        & \multicolumn{1}{c|}{0.720}        & 0.649                             & 0.621          & 0.636         & 0.668          & \multicolumn{1}{c|}{0.745}        & 0.668                            \\
\textbf{Accuracy}  & 0.740         & 0.711         & 0.718        & \multicolumn{1}{c|}{0.697}          & 0.717                                       & 0.713         & 0.683         & 0.695        & \multicolumn{1}{c|}{0.682}        & 0.693                             & 0.715          & 0.691         & 0.680          & \multicolumn{1}{c|}{0.679}        & 0.691                            \\
\textbf{F1}        & 0.634         & 0.645         & 0.694        & \multicolumn{1}{c|}{0.686}          & 0.665                                       & 0.614         & 0.629         & 0.686        & \multicolumn{1}{c|}{0.684}        & 0.653                             & 0.603          & 0.634         & 0.647          & \multicolumn{1}{c|}{0.662}        & 0.637                           
\end{tabular}}
\caption{Performance of NLI and LLM based adequacy classifiers on manually annotatated examples for four different models.}
\label{tab:adeq_classifiers}
\end{table*}

In order to decide for the optimal $a(\cdot;\lambda)$, we evaluate the classifiers using the manually annotated outputs. For each OPT-model, we assess accuracy, precision, recall and F1-score on 500 annotations (50 contexts x 10 generations). 
Using the optimal method, we perform a large-scale evaluation using all 741 ambiguous instances from Abg-COQA's training set, all 253 ambiguous and 253 (randomly sampled) non-ambiguous instances from the development and testing set.% (not used for any decisions' optimisation).
%analysis similar to before, \emph{i.e.} 10 generated samples are used to compute AP for OPT2.7B-30B and assess its performance using AUROC as an evaluation metric, against Semantic Entropy and Predictive entropy and their normalised counterparts --- on the same dataset subset. 
 %To further asses the validity of our metric, we repeat a similar analysis on a subset of the Abg-COQA's development and test set (which was not previously used for any evaluation before). This comprises 253 ambiguous instances, and we randomly sample the same number of unambiguous instances.
%As such, we assess the usefulness of our method when generalising to new instances and a setting where a mix of low and high ambiguity instances are present.


